LMGQS: A Large-scale Dataset for Query-focused Summarization

Query-focused summarization (QFS) aims to extract or generate a summary of an input document that directly answers or is relevant to a given query. The lack of large-scale datasets in the form of documents, queries, and summaries has hindered model development in this area. In contrast, multiple large-scale high-quality datasets for generic summarization exist. We hypothesize that there is a hidden query for each summary sentence in a generic summarization annotation, and we utilize a large-scale pretrained language model to recover it. In this way, we convert four generic summarization benchmarks into a new QFS benchmark dataset, LMGQS, which consists of over 1 million document-query-summary samples. We thoroughly investigate the properties of our proposed dataset and establish baselines with state-of-the-art summarization models. By fine-tuning a language model on LMGQS, we achieve state-of-the-art zero-shot and supervised performance on multiple existing QFS benchmarks, demonstrating the high quality and diversity of LMGQS.

==> tables/mds_res.bak.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[ht]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}c|l|lll|lll|lll@{}}
\toprule
\multicolumn{1}{l|}{} &
   &
  \multicolumn{3}{c|}{DUC 2006} &
  \multicolumn{3}{c|}{DUC 2007} &
  \multicolumn{3}{c}{TD-QFS} \\ \midrule
\multicolumn{1}{l|}{Category} &
  Model &
  R-1 &
  R-2 &
  R-L &
  R-1 &
  R-2 &
  R-L &
  R-1 &
  R-2 &
  R-L \\ \midrule
\multirow{4}{*}{Upper Bound \&   Baselines} &
  Gold &
  45.4 &
  11.2 &
  16.8 &
  47.5 &
  14 &
  18.9 &
  52.2 &
  27 &
  30.2 \\
 &
  Oracle &
  47.5 &
  15.8 &
  20.2 &
  47.6 &
  17.1 &
  20.9 &
  64.9 &
  48.3 &
  49.4 \\
 &
  Lead &
  32.1 &
  5.3 &
  10.4 &
  33.4 &
  6.5 &
  11.3 &
  33.5 &
  5.2 &
  10.4 \\
 &
  LexRank &
  34.2 &
  6.4 &
  11.4 &
  35.8 &
  7.7 &
  12.7 &
  35.3 &
  7.6 &
  12.2 \\ \midrule
\multirow{3}{*}{Distantly Supervised} &
  QuerySum &
  41.6 &
  9.5 &
  15.3 &
  43.3 &
  11.6 &
  16.8 &
  44.3 &
  16.1 &
  20.7 \\
 &
  Bart-CAQ &
  38.3 &
  7.7 &
  12.9 &
  40.5 &
  9.2 &
  14.4 &
  — &
  — &
  — \\
 &
  PQSum &
  40.9 &
  9.4 &
  14.8 &
  42.2 &
  10.8 &
  16 &
  — &
  — &
  — \\ \midrule
\multirow{6}{*}{Few- or Zero-shot   Abstractive} &
  MARGESUM &
  40.2 &
  9.7 &
  15.1 &
  42.5 &
  12 &
  16.9 &
  45.5 &
  16.6 &
  20.9 \\
 &
  BART &
  38.3 &
  7.8 &
  13.1 &
  40.2 &
  9.9 &
  14.6 &
  45.1 &
  16.9 &
  21.4 \\
 &
  GSUM+LEXRANK &
  38.1 &
  7.9 &
  13.1 &
  39.5 &
  9.5 &
  14.3 &
  45.5 &
  18.0 &
  22.4 \\
 &
  LQSUM &
  39.1 &
  8.5 &
  13.7 &
  40.4 &
  10.2 &
  15 &
  \textbf{45.7} &
  \textbf{18.1} &
  \textbf{22.1} \\
 &
  CNN/DM BART &
  39.3 &
  8.5 &
  13.5 &
  39.9 &
  10.0 &
  14.5 &
  39.7 &
  9.9 &
  15.1 \\
 & \DatasetNameSpace BART & \textbf{41.1} & \textbf{9.3} & \textbf{14.8} & \textbf{41.1} & \textbf{10.7} & \textbf{15.6} & 41.6 & 11.8 & 16.9 \\ \bottomrule
\end{tabular}%
}
\caption{ROUGE scores on multi-document QFS dataset DUC 2006, DUC2007.}
\label{tab:mds_res}
\end{table*}
